Going with the flow: using gas clouds to probe the accretion flow feeding Sgr A*

The massive black hole in our galactic center, Sgr A*, accretes only a small fraction of the gas available at its Bondi radius. The physical processes determining this accretion rate remain unknown, partly due to a lack of observational constraints on the gas at distances between ~10 and ~10$^5$ Schwarzschild radii (Rs) from the black hole. Recent infrared observations identify low-mass gas clouds, G1 and G2, moving on highly eccentric, nearly co-planar orbits through the accretion flow around Sgr A*. Although it is not yet clear whether these objects contain embedded stars, their extended gaseous envelopes evolve independently as gas clouds. In this paper we attempt to use these gas clouds to constrain the properties of the accretion flow at ~10$^3$ Rs. Assuming that G1 and G2 follow the same trajectory, we model the small differences in their orbital parameters as evolution resulting from interaction with the background flow. We find evolution consistent with the G-clouds originating in the clockwise disk. Our analysis enables the first unique determination of the rotation axis of the accretion flow: we localize the rotation axis to within 20 degrees, finding an orientation consistent with the parsec-scale jet identified in x-ray observations and with the circumnuclear disk, a massive torus of molecular gas ~1.5 pc from Sgr A*. This suggests that the gas in the accretion flow comes predominantly from the circumnuclear disk, rather than the winds of stars in the young clockwise disk. This result will be tested by the Event Horizon Telescope within the next year. Our model also makes testable predictions for the orbital evolution of G1 and G2, falsifiable on a 5-10 year timescale.

==> table/table.tex <==
% table.tex: split this off into its own file, since it's pretty
% long.
%
% load it into the main document with \input{table/table.tex}.
% test it by compiling the included test-table.tex
%
% this table requires the following packages to be loaded:
% 
%  1. textcomp
%  2. [utf8]{inputenc}
%  3. booktabs
%  4. multirow
%  5. threeparttable
% 
% I think all of these are included in standard tex distributions

% this table is kind of a bear... there are two layers of complexity:
%
% - first, I use the threeparttable package to get a caption, table,
%   tablenotes layout.  this is so we can explain why/how we split the
%   G2 data into two different measurements
%
% - second, I align the data columns at both the decimal points and
%   the ± signs.  so each of these columns is really FOUR columns,
%   with the structure #,.,#,±,#,.,#, where the four #'s are the four
%   columns of digits.  phew!
%
\begin{table*}
\centering
\begin{threeparttable}
%
%
\caption{Published Kepler elements we use to constrain our models.
  Numbers in the first group represent measurements very close to G2's
  pericenter passage.  Numbers in the second group come from earlier
  studies; these provide a hint of evolution in G2's orbital elements,
  but may have larger uncertainties.  We perform our analysis both
  with and without this second group.  Empty cells are not used in our
  fits.  TODO: add omega.  also add our fits from the appendix\ldots
  how do we stack up?}\label{tab:obs-kepler}
%
%
\begin{tabular}
{r@{.}l%
r@{.}l@{\;±\;}r@{.}l% #, decimal, #, ±, #, decimal, #
r@{.}l@{\;±\;}r@{.}l%
r@{.}l@{\;±\;}r@{.}l%
r@{.}l@{\;±\;}r@{.}l}
%
\toprule 
%% heading
%  - first column is time and spans *two* columns
%  - columns with data actually span *four* columns
%
\multicolumn{2}{c}{year (JD)}
& \multicolumn{4}{c}{$a$\,('')}
& \multicolumn{4}{c}{$e$}
& \multicolumn{4}{c}{$i$\,(°)}
& \multicolumn{4}{c}{$\Omega$} \\
\midrule
%
%% G1 data
%  - each line is a datapoint, which is 4 columns to latex
%  - on each line, &'s stand in for decimal points and for the ±
%    sign.  sorry this is hard to read
\multicolumn{2}{c}{(free)\tnote{1}}
&   0&36 & 0&16  % a
&   0&86 & 0&05  % e
& 108&0  & 2&0   % i
&  69&0  & 5&0   % Ω
\\
%
%% G2 data
2013&33\tnote{2}
&   1&05  & 0&25  % a
&   0&976 & 0&007 % e
& 118&0   & 2&0   % i
&  82&0   & 4&0   % Ω
\\
\midrule 
%
%% put non-obvious things here, separate from things directly copied
%% from Pfuhl.  each of these needs a footnote explaining what we do.
%
%% G2 data
2012&56\tnote{3}
& \multicolumn{4}{c}{   } % a
&   0&981 &  0&006        % e
& 121&0   &  3&0          % i
&  56&0   & 11&0          % Ω
\\
%
2012&42\tnote{4}
& \multicolumn{4}{c}{   } % a
&   0&966  & 0&003        % e
& 109&5    & 0&8          % i
&  95&8    & 1&1          % Ω
\\
2011&00\tnote{5}
& \multicolumn{4}{c}{   } % a
& 0&938  & 0&007          % e
& \multicolumn{4}{c}{   } % i
& \multicolumn{4}{c}{   } % Ω
\\
\midrule
\multicolumn{2}{c}{$-\infty$\tnote{6}}
& \multicolumn{4}{c}{   } % a
& \multicolumn{4}{c}{   } % e
& 126&0  &  20&9          % i
&  98&0  &  18&0          % Ω
\\
%
\bottomrule
%
\end{tabular}
%
%
\begin{tablenotes}
\item [1] Pfuhl et al. 2014.  Following these authors, we assume G1
  follows the same orbital trajectory as G2.  We allow the time
  difference between G1 and G2 to float as part of our parameter
  optimization.
%
\item [2] Gillessen et al. 2013b
%
\item [3] Phifer et al. 2013.  {\color{red!80!black}{Pfuhl
  indicates this is more representative of 2014.5\ldots why the
  difference?}}
%
\item [4] Gillessen et al. 2013a
%
\item [5] Gillessen et al. 2012a
%
\item [6] G2's energy and inclination suggest that it may have
  originated in the stellar disk.  We therefore include this as a data
  point near the apocenter of G2's orbit.  Since this origin for G2 is
  uncertain, we perform our analysis with and without this extra
  constraint.  Inclination taken from Bartko et al. (2009).
%
\end{tablenotes}
%
%
\end{threeparttable}
\end{table*}

%% Local Variables:
%% compile-command: "rubber -df --warn all test-table.tex && open test-table.pdf"
%% End:

